Long Plane Trees

In the longest plane spanning tree problem, we are given a finite planar point set $\mathcal{P}$, and our task is to find a plane (i.e., noncrossing) spanning tree for $\mathcal{P}$ with maximum total Euclidean edge length. Despite more than two decades of research, it remains open whether this problem is NP-hard. Thus, previous efforts have focused on olynomial-time algorithms that produce plane trees whose total edge length approximates $\text{OPT}$, the maximum possible length. The approximate trees in these algorithms all have small unweighted diameter, typically three or four. It is natural to ask whether this is a common feature of longest plane spanning trees, or an artifact of the specific approximation algorithms. We provide three results to elucidate the interplay between the approximation guarantee and the unweighted diameter of the approximate trees. First, we describe a polynomial-time algorithm to construct a plane tree with diameter at most four and total edge length at least $0.546 \cdot \text{OPT}$. This constitutes a substantial improvement over the state of the art. Second, we show that a longest plane tree among those with diameter at most three can be found in polynomial time. Third, for any candidate diameter $d \geq 3$, we provide upper bounds on the approximation factor that can be achieved by a longest plane tree with diameter at most $d$ (compared to a longest plane tree without constraints).

==> sec-dp-triangle.tex <==
% !tex root=./main-arxiv.tex
\subsection{Extending the approach to special trees of diameter 4}
Now we show how we can extend the ideas to get a polynomial time algorithm for a more general situation.
Given three points \(a,b,c\), a \emph{tristar} rooted at \(a,b\) and \(c\) is a tree, where all points are connected to either \(a,b\) or \(c\). 
We will now argue that we can compute the best tristar rooted at a triple of points on the boundary of the convex hull in polynomial time.

As in \cref{subsec:dpbistar} we will use dynamic programming. However, before we can use the dynamic programming approach we have to do some precomputing steps.

Assume that both \(a, b\) and \(c\) and the edges incident to two of these vertices are fixed. Without loss of generality assume that \(a\) and \(b\) lie on a horizontal line and that the fixed edges are \(ac\) and \(bc\).
Note that everything cut off by the edges \(ac\) and \(bc\) is independent of the rest and can be solved by using the dynamic program described in \cref{subsec:dpbistar}, see \cref{fig:tristarexclude}.
So now we only consider the remaining part of the point set.

\begin{figure}[h]
\centering
\includegraphics{figures/tristarexclude.pdf}
\caption{The light blue regions are independent from the remaining problem.}
\label{fig:tristarexclude}
\end{figure}

So now assume that in addition to the fixed \(a\) and \(b\), we also correctly guessed the highest points \(p\) and \(q\) such that \(p\) is connected to \(a\) and \(q\) is connected to \(b\). Now that these edges are fixed, the current region decomposes into subregions, depending on which of the three roots are visible from within the regions. See \cref{fig:tristarregions} for an illustration. We call the choice of \(a,b,c,p\) and \(q\) together with the edges within \(\{a,b,c\}\) a \emph{starting configuration}. We now describe how to solve the problem for a fixed starting configuration.


\begin{figure}[h]
\centering
\includegraphics{figures/tristarregions.pdf}
\caption{The edges \(ap\) and \(bq\) subdivide the current region into visibility regions.}
\label{fig:tristarregions}
\end{figure}

Note that edges from points below \(p\) and above the edge \(ap\) do not interfere with any other edges, so we can again find an optimal solution for these by using the dynamic program from \cref{subsec:dpbistar}. We can also already add the edges to regions only visible from or feasible for one vertex.

Next we want to fix the edges in the horizontal strip defined by \(p\) and \(q\). We again guess a point. This time we guess the point \(k\) with largest \(x\)-coordinate which is connected to \(a\). This redefines the center region as can be seen in \cref{fig:tristarmiddle}.

\begin{figure}[h]
\centering
\includegraphics[page=2]{figures/tristarmiddle.pdf}
\caption{Fixing the rightmost point \(k\) connected to \(a\) gives easier to handle regions.}
\label{fig:tristarmiddle}
\end{figure}

Now the part bounded by the vertical line through \(k\) and the region above the edge \(ak\) is again independent from the remaining regions and can be solved by using the dynamic program from above with roots \(a\) and \(c\). By a similar argument the parts above the edge \(qb\) are either uniquely determined to connect to \(b\) or are also independent from the remaining points and can thus be connected optimally by the dynamic program from above.
 Finally the remaining regions of the strip between \(p\) and \(q\) are uniquely determined and can therefore also been put into place.

Let \(r\) be the lowest point connected  to \(c\) in the horizontal strip between \(p\) and \(q\). Furthermore redefine \(p\) to be the lowest point below the edge \(ak\) but above the horizontal line through \(q\). Note that the triangle \(\Delta pqr\) does not contain any points and that all points above of the edges \(pa\) and \(qb\) are already, independently of the remaining points, connected to some point.

Keeping the invariant that \(\Delta pqr\) is empty and that the points above the edges \(ap\) and \(bq\) are fixed we can now go to defining the dynamic programming part of our solution. 
The basic idea is similar to the dynamic program above. Given three points \(p,q,r\) such that the edges \(ap\), \(bq\) and \(cr\) are fixed, and the triangle \(\Delta pqr\) is empty, we want define \(P_{pqr}\) to be best spanning tree for the points in the truncated triangle defined by \(ap\) and \(bq\) and below the lowest point \(m\) of the three points.
Let \(k\) be the highest point in the truncated triangle which lies below \(m\). If no such \(k\) exists, the value is simply \(0\). In the other case it can be determined recursively. See \cref{fig:tristarrecurrence} for the definition of the regions \(A, A', B\) and \(B'\).
\begin{align*}
 P_{pqr}&=\max \begin{cases}
 P_{kqr} + \Vert ak \Vert + \mathrm{OPT}(A) + \sum_{l\in A'} \Vert la \Vert\\
 P_{pkr} + \Vert bk \Vert + \mathrm{OPT}(B) + \sum_{l\in B'} \Vert lb \Vert \\
 P_{pqk} + \Vert ck \Vert& \text{if } k \text{ is visible from } k
 \end{cases}
 \end{align*} 
 Where \(A\) and \(B\) are again regions which are independent of the points which are still to be considered, so we can again use the dynamic program from \cref{subsec:dpbistar} to solve them.

 \begin{figure}
 \centering
 \includegraphics{figures/tristarrecurrence.pdf}
 \caption{The different cases for the recurrence}
 \label{fig:tristarrecurrence}
 \end{figure}

 To then get the overall optimal solution for fixed \(a,b\) and \(c\), the fixed edges between them and the fixed highest points connected to \(a\) or \(b\), we simply sum up the fixed edges from the preprocessing, the solution of \(P_{pqr}\) and the length of the edges \(ap\) and  \(bq\).

 To find the overall best tristar we have to iterate over all possible triples on the convex hull and all possible edges between them. These are \(O(n^3)\) possibilities. For each of these possibilities we fix the two vertices above the non edge pair which are the highest. These are additional \(O(n^2)\) possible pairs. Furthermore we have to fix the rightmost \(k\) connected to \(a\) in the horizontal strip. So we run the program above for \(O(n^6)\) possible starting configurations.

  Filling out the table costs \(O(n^3)\) plus the time needed to compute the \(\mathrm{OPT}(A)\), so in a rough estimate overall \(O(n^5)\). The preprocessing steps also take a total of at most \(O(n^2)\) so overall we have \(O(n^5)\) running time for a fixed configurations.
 As this is needed for all \(O(n^6)\) starting configurations, we get a total running time of \(O(n^{11})\) which is polynomial.

\katharina{We can probably this to \(O(n^4\) or even \(O(n^3)\) for filling out the table by considering how often each point is part in a \(O(n^2)\) independent computation.}

\katharina{It is well possible that this idea could also be more or less easily extended to arbitrary tristars and not only those on the convex hull}
